Decidability of Quasi-Dense Modal Logics

The decidability of axiomatic extensions of the modal logic K with modal reduction principles, i.e. axioms of the form $\Diamond^{k} p \rightarrow \Diamond^{n} p$, has remained a long-standing open problem. In this paper, we make significant progress toward solving this problem and show that decidability holds for a large subclass of these logics, namely, for 'quasi-dense logics.' Such logics are extensions of K with with modal reduction axioms such that $0 < k < n$ (dubbed 'quasi-density axioms'). To prove decidability, we define novel proof systems for quasi-dense logics consisting of disjunctive existential rules, which are first-order formulae typically used to specify ontologies in the context of database theory. We show that such proof systems can be used to generate proofs and models of modal formulae, and provide an intricate model-theoretic argument showing that such generated models can be encoded as finite objects called 'templates.' By enumerating templates of bound size, we obtain an EXPSPACE decision procedure as a consequence.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> old-06-ExistentialRules.tex <==
\section{Existential Rules and Decision Procedure}\label{sec:erules}

\begin{definition}
    Let $\sig$ denote the following signature:
    $$\set{\ppred_\Psi \mid \Psi \text{ is a $\theform$-subformula } \theform \text{ or its negation}} \cup \set{\epred, \rpred, \goal} \cup \set{\dpred_i \mid i \in [0,n]}$$
    where all symbols are unary with the exception of $\epred$ and $\rpred$.
\end{definition}

\begin{definition}
    Let $\rsa$ be the ruleset having the following rule per each $k \rightarrow \kp \in \axioms$:
    \begin{align*}
    \arule{\epred(x_0, x_1)\ldots\epred(x_{k-1}, x_k)}{y_1, \ldots y_{\kp - 1}}{\epred(x_0, y_1), \epred(y_{\kp -1}, x_k)}.
    \end{align*}
\end{definition}

\begin{definition}
    A \emph{selection formula} $\select_i(x)$ of depth $i$ is the following formula:
    $$\bigwedge \ppred_{\Psi}(x) \lor \ppred_{\neg\Psi}(x)$$
    where $\Psi$ ranges over symbols of $\subform_i(\theform)$.
\end{definition}


\begin{definition}
    Given a set of natural numbers $X$ and a density axiom $\kkp$ we define $\kkp(X)$ containing each element of $X$ as well as each $j \leq n$ such that there is a natural number $i \in X$ satisfying $i \geq k$ and $j = i + \kp - k$. We denote the fix-point of such operation with $\kkp^*(X)$. We extend this operation to work with sets of density axioms denoted with $\axioms(X)$.
\end{definition}

\begin{definition}
    A \emph{depth formula} $\depths_i(x)$ of depth $i$ is the following formula:
    $$\bigwedge_{j \in \axioms^*(\set{i})} \dpred_j(x).$$
\end{definition}

\begin{definition}
    Let $\rsp$ be the ruleset consisting of the following rules:
    \begin{align*}
        \adrule{\dpred_{i}(x)}{\depths_i(x)}\tag{i}\label{tag:depths-closure}\\
        \adrule{\dpred_i(x)}{\select_i(x)}\tag{ii}\\
        \adrule{\dpred_{i}(x) \land \epred(x, y)}{\dpred_{i + 1}(y)}\tag{iii}\label{tag:depths-propagation}\\
        \narule{\ppred_{\mlbox\Psi}(x)\land \dpred_{i}(x)}{y}{\dpred_{i + 1}&(y) \land \ppred_{\Psi}(y) \land \epred(x,y) \land \rpred(x, y)}\tag{iv}\\
        \adrule{\ppred_{\Psi \land \Psi'(x)}}{\ppred_{\Psi}(x) \lor \ppred_{\Psi'}(x)}\tag{v}\\
        \adrule{\ppred_{\Psi \lor \Psi'(x)}}{\ppred_{\Psi}(x) \land \ppred_{\Psi'}(x)}\tag{vi}\\
        \adrule{\ppred_{\mldia\Psi}(x)\land\epred(x,y)\land\ppred_{\neg\Psi}(y)\land\ppred_{\theform}(z)}{\goal(z)}\tag{vii}\\
        \adrule{\ppred_{\Psi}(x) \land \ppred_{\neg \Psi(x)} \wedge \ppred_{\theform}(y)}{\goal(y)}\tag{viii}
    \end{align*}
    for $i \in [0,n]$ and $\Psi$ ranging over sub-formulae of $\theform$.
\end{definition}

\noindent
Finally
\begin{definition}
    Let $\dbz$ be the database $\set{\dpred_0(a)}$ for a constant $a$.
\end{definition}

\noindent
The following is straightforward:

\begin{observation}
    $\rsa \cup \rsp, \dbz \models \goal(a)$ \iffi \piotr{proof search always derives $\bot$}
\end{observation}
\begin{proof}
    \piotr{Needs the former section to even attempt proving it.}
\end{proof}

\noindent
Thus, in order to prove Theorem~\ref{thm:main}
it is enough to show the following lemma:

\begin{lemma}\label{lem:existential-decidability-problem}
    Verifying $\rsa \cup \rsp, \dbz \models \goal(a)$ is decidable.
\end{lemma}

\noindent
\subsection{Proof of Lemma~\ref{lem:existential-decidability-problem}}
For the rest of this paper, let $\chases$ be the set of all chases of $\rsp \cup \rsa$ over $\dbz$.

\begin{definition}[$\unfold$]\label{def:unfold}
Given an instance $\inst$ with no infinite paths, one of its terms $t$ and a word $a$ over the set of terms, we define $\unfold(\inst, t, a)$ inductively as follows:
\begin{equation*}
    \unfold(\inst, t, a) = \labels(t)[t \mapsto at] \cup \bigcup_{\alpha(t, s) \in \inst} \alpha(at, ats) \bigcup_{s \in \esucc(t)} \unfold(\inst, s, at) 
\end{equation*}
Note that the recursion halts for all paths in $\inst$. We will write $\unfold(\inst)$ meaning $\unfold(\inst, r, \varepsilon)$ if $r$ is the only maximal term of $\inst$.
\end{definition}


\begin{definition}[$\trim$]\label{def:trim}
Given a multi-tree $\tree$ over $\set{\epred, \rpred}$ and a natural number $n$, we define $\trim_n(\tree)$ as the tree $\tree$ with all the elements past depth $n$ removed, except for the elements reachable with $R$-paths from elements at depths not larger than $n$.
\end{definition}



\begin{definition}[$\spairs$]\label{def:spair}
    Given an instance $\inst$ 
    a \emph{successor pair} $\spair(t, t)$ is an instance formed from two terms $t$ and $t'$ of $\inst$ and all atoms mentioning only those two terms.

    We define the \emph{successor type} $\spairs(\inst)$ of $\inst$ as the set $\set{\spair(s_0, s_1) \mid \spair(t, t') \text{ is a successor pair of } \inst}$ where $s_0$ and $s_1$ are two special constants.
\end{definition}


\begin{definition}[$\embed$]\label{def:embed}
    Given a tree $\tree$ and two of its terms $t$ and $t'$ such that there is a homomorphism $h$ from $\tree_t$ to $\tree_{t'}$ we write $\embed(\tree, t, t', h)$ to indicate an instance $\bar{h}(\tree)$ where $\bar{h}$ is an extension of $h$ over the set of all terms that is an identity outside of the domain of $h$.
\end{definition}

\begin{definition}
    Given a density axiom $\kkp$, a tree $\tree$ and one of its terms $t$, we say that $t$ is $(\kkp)$-\emph{compliant} \iffi 
    for every descendant term $t'$ of $t$ at a distance $k$ there exists a descendant term $t_+$ of $t$ at a distance $\kp$ such that $\tree_{t_+}$ is homomorpically mappable to $\tree_{t'}$ through a homomorphism $h$. We call every such $\pair{t', t_+, h}$ a \emph{compliance witness} for $t$. 
    We extend this notion to sets of density axioms in a natural way.
\end{definition}

In order to decide the entailment stated in Lemma~\ref{lem:existential-decidability-problem} we will show that the information within the chase can be represented through a finite object called a {\em map}. We define the set of properties such an object should satisfy below, but encourage the reader to briefly skim through the rest of this section to understand how maps will be used to prove Lemma~\ref{lem:existential-decidability-problem}.

\begin{definition}\label{def:map}
    A \emph{map} $\map$ is an instance that satisfies the following properties:
    \begin{enumerate}
        \item $\map$ is a tree such that $\trim_N(\map) = \map$.  \label{map:trim-id-on-map}
        \item Every term of $\map$ at depth no greater than $n$ is $\axioms$-compliant.  \label{map:shallow-compliance}
        \item $\map$ is a model of $\rsp$. \label{map:modelhood}
        \item $\map$ is a core. \label{map:cored}
        \item For all $t', t_+, h$ that are witnessing $A$-compliance of $t$ at depth no greater than $n$ in $\map$ the following holds:
        $\core \circ \trim_N \circ \unfold \circ \embed(\map, t_+, t', h)$ is isomorphic to $\map$. \label{map:embedding-and-unfolding}
        \item The root of $\map$ is labelled with $\dpred_0$. \label{map:phi-at-root}
        \item $\map$ with any label removed is not a model of $\rsp$.\label{map:minimality}
    \end{enumerate}
\end{definition}

The above definition might seem complex, but it is meant to avoid numerous pitfalls uncovered while designing Lemma~\ref{lem:map-to-chase} and its proof.


\begin{observation}\label{obs:chase-to-map}
For any $\ch \in \chases$ we have $\map = \core \circ \trim_N \circ \unfold(\ch)$ is a map. Moreover $\spairs(\map) \subseteq \spairs(\ch)$.
\end{observation}
\begin{proof}
We shall go over the properties:
\begin{enumerate}
    \item By the definitions of $\trim$ and $\core$.
    \item By the definition of $\unfold$ and $\trim$.
    \item Note that $\spairs(\map) \subseteq \ch$, this shows that the Datalog rules of $\rsp$ are satisfied. By the definition of $\trim$ we note that all non-Datalog rules of $\rsp$ are satisfied as well.
    \item Trivial.
    \item By the definition of $\trim$ and $\unfold$. 
    \item Trivial.
    \item Trivial.
\end{enumerate}
The last assertion $\spairs(\map) \subseteq \ch$ is trivially satisfied by definition of $\trim$, $\unfold$ and $\core$.
\end{proof}

\begin{lemma}\label{lem:map-to-chase}
    For every map $\map$ there exists a chase $\ch \in \chases$ such that $\spairs(\ch) \subseteq \spairs(\map)$.
\end{lemma}

We shall prove the above lemma in the next section. Before that, let us see how to use it in the proof. From Observation~\ref{obs:chase-to-map} and Lemma~\ref{lem:map-to-chase} we have:

\begin{corollary}
    There exists a map $\map$ such that $\goal(a) \not\in \map$ \iffi there exists a chase $\ch \in \chases$ such that $\goal(a) \not\in \ch$.
\end{corollary}

One can leverage the above to decide whether $\chases \models \goal(a)$ by enumerating all the maps (there is a finite number of those that we have to consider) and checking whether there exists one that does not contain $\goal$. Thus we get:

\begin{corollary}
    It is decidable to check whether $\rsp, \rsa, \dbz \models \phi$.
\end{corollary}

The above corollary is in fact Lemma~\ref{lem:existential-decidability-problem}. Thus we would get Theorem~\ref{thm:main}.

\subsection{Proof of Lemma~\ref{lem:map-to-chase}}

By inspecting the rules of $\rsp \cup \rsa$ we note:
\begin{observation}\label{obs:chase-has-minimal}
    Every element of $\chases$ has single minimal term - that is a term with no incoming edges.
\end{observation}

Given an instance $\inst$ and any trigger $\pi$ of $\rsa$ in $\inst$ let $\iter(\inst, \pi)$ denote the set of instances resulting from the application of the following two-part operation: 

\begin{enumerate}
    \item Apply $\pi$.
    \item Saturate with rule applications of Datalog rules of $\rsp$.
\end{enumerate}

\noindent
Given an instance $\inst$ and any trigger $\pi$ of some non-Datalog rule of $\rsp$ in $\inst$ let $\iterr(\inst, \pi)$ denote the set of instances resulting from the application of the following two-part operation: 

\begin{enumerate}
    \item Apply $\pi$.
    \item Saturate with rule applications of Datalog rules of $\rsp$.
\end{enumerate}

First note that any chase of $\chases$ can be obtained by looping the following two operations and selecting an element of the resulting set each time.

\begin{lemma}\label{obs:proof-of-main-lema-a}
Given an instance $\inst$ and a map $\map$
if $\core \circ \trim_N \circ \unfold(\inst)$ homomorphically maps to $\map$ then for every $\rsa$-trigger $\pi$ in $\inst$ there exists $\inst' \in \iter(\inst, \pi)$ such that $\core \circ \trim_N \circ \unfold(\inst')$ homomorphically maps to $\map$.

\end{lemma}
\begin{proof}

Let $\jnst = \core \circ \trim_N \circ \unfold(\inst)$. Then let $\inst_{0}$ to be the result of applying $\pi$,  $P$ be the path from $t$ to $t'$ witnessing that $\pi$ was not satisfied in $\inst$, and $P_+$ be the freshly created path. Finally let $k \rightarrow \kp$ be the existential rule of $\pi$.

If $t$ has no label then it appears in the chase at depth greater than $n$. Therefore, the observation holds trivially as all successors of $t$ including all new elements of $P'$ are removed by $\trim$ function before homomorphic mapping is considered, thus the homomorphism from assumption can be reused.

Assume that $t$ has a label, and thus is at depth $d \leq n$.
Let $u'$ be the term of $\jnst$ such that the shortest path from the minimal (recall Observation~\ref{obs:chase-has-minimal}) term of $\inst$ to $t'$ is isomorphic to the path from the root of $\jnst$ to $u'$, and let $u$ be the predecessor of $u'$ at distance $k$ from $u$. Note that by the definitions of $\core, \trim$, and $\unfold$ operations such $u$ and $u'$ exist. Let $h$ be the homomorphism from $\jnst$ to $\map$ and let $v = h(u), v' = h(u')$.

As $u$ is at depth $d$ Property~\ref{map:shallow-compliance} of the map can be applied. Let $w = \pair{h, u', u_+}$ be the $(k \rightarrow \kp)$-compliance witness for $u$. We want to construct a basis $\inst_+$ for the required $\inst'$. To do that we take $\inst_0$ and consecutively copy labels from the path from $u$ to $u_+$ over the elements of $P_+$. We set $\inst_{+}$ to be the resulting instance. Thanks to Properties~\ref{map:embedding-and-unfolding} and ~\ref{map:modelhood} of the map, and the existence of $w$ it should be clear that $\core \circ \trim_N \circ \unfold(\inst_+)$ homomorphically maps to map $\map$. Again, such constructed $\inst_+$ will serve us as a basis for $\inst'$.

First note, that the depth-labels over $P_+$ are the same in any element of $\iter(\inst, \pi)$. This is thanks to (\ref{tag:depths-closure}) and (\ref{tag:depths-propagation}) rules of $\rsp$. Thus from Property \ref{map:minimality} of the map the same labels as on path from $u$ to $u_+$ can be ``guessed'' by $\rsp$. Observe that in $\iter(\inst, \pi)$ there is only one such instance - as the only disjunctive rules of $\rsp$ are those guessing the labels of terms. Thus, instances $\inst_{+}$ and $\inst_{\iter}$ can in principle differ only by a special, single atom, namely $\goal(a)$. 

There are four cases depending of whether $\goal(a)$ is present in map $\map$ and whether it is was just derived in $\inst_\iter$. If $\goal(a) \in \map$ then no matter whether $\goal(a) \in \inst_\iter$ or not, $\inst_\iter$ is homomorphically mappable to $\map$ and thus it can serve as $\inst'$.

Assume that $\goal(a) \not\in \map$. If $\inst_\iter$ does not contain $\goal(a)$ then it is homomorphically mappable to $\map$ as $\inst_{+}$ is. Thus $\inst_\iter$ can serve as $\inst'$.

Finally assume that $\goal(a) \not \in \map$ but $\goal(a) \in \inst_\iter$. However, note that $\chase{\inst_0, \rsp} = \inst_\iter$, $\map$ is a model of $\rsp$, and $\spairs(\inst_0) \subseteq \spairs(\map)$, but $\goal(a) \not \in \map$. This is a contradiction by \piotr{Lemma stating that violations of modelhood of $\rsp$ can be witnessed by a single spair.}
\end{proof}

The following is proven analogously:

\begin{observation}\label{obs:proof-of-main-lema-b}
Given an instance $\inst$ and a map $\map$
if $\core \circ \trim_N \circ \unfold(\inst)$  homomorphically maps to $\map$ then for every non-Datalog trigger $\pi$ of $\rsp$ in $\inst$ there exists $\inst' \in \iter(\inst, \pi)$ such that $\core \circ \trim_N \circ \unfold(\inst')$ homomorphically maps to $\map$.
\end{observation}
\begin{proof}
\piotr{TODO if time - this one is boring.}

One can inductively combine the above to obtain Lemma~\ref{lem:map-to-chase}.

\end{proof}



\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OLD STUFF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
    Given an acyclic instance $\inst$ with $a$ being its source node, and a map $\map$ if $\core \circ \trim_N \circ \unfold(\chase{\inst, \rsd})$ homomorphically maps to $\map$ then for every $\rsp \cup \rsa$ trigger $\pi$ in $\inst$ there exists $\inst' \in \apply{\inst, \pi}$ such that $\core \circ \trim_N \circ \unfold(\chase{\inst', \rsd})$ homomorphically maps to $\map$.
\end{lemma}
\begin{proof}
    Let $\pi = \pair{\rho, f}$, $\jnst = \core \circ \trim_N \circ \unfold(\chase{\inst, \rsd})$, and $h$ be the homomorphism from $\jnst$ to $\map$.
    
    Assume $\rho \in \rsp$. Note that as map $\map$ is a model of $\rsp$ thus there are no active triggers in it for any rule of $\rsp$. Thus $\chase{\map, \rsp} = \map$. If $\rho$ is non-disjunctive then the rest follows from Observation~\ref{obs:chase-preserves-homs}. Assume that $\rho$ contains disjunction in its head and thus is one of (\ref{rule:head-disjunction}) rules. Let $t = f(x)$ for $x$ as in (\ref{rule:head-disjunction}). Let $P_t$ denote the path in $\inst$ from its source to $t$, note that the term $\word(P_t)t$ was not trimmed-out in $\jnst$. We know this as $t$ has a label and thus $|word(P_t)t| \leq n$. Let $u$ denote $\word(P_t)t$. As $\jnst \rightarrow \map$ we know that $\body{\rho}(h(u)) \in \map$ thus there exists a trigger $\pi' = \pair{\rho, x \mapsto h(u)}$ in $\map$. However, as $\map$ is a model of $\rsp$ we know that $\pi'$ is satisfied by some atom $\alpha(h(u)) \in \head{\rho}$. Now we can simply add $\alpha(t)$ to $\inst$ during application of $\pi$ and set $\inst'$ to be the resulting instance. Note that $h$ is a homomorphism from $\core \circ \trim_N \circ \unfold(\inst')$ to $\map$.

    Assume $\rho \in \rsa$. As maps are not inherently models of $\rsa$, we cannot use the above to reasoning in this case. Let $\inst'$ to be the result of applying $\pi$, $P$ be the path from some $t$ to $t'$ witnessing that $\pi$ was not satisfied in $\inst$, $P_+$ be the freshly created path, $P_t$ be the shortest path from the source of $\inst$ to $t$, and $k \rightarrow \kp$ the density axiom giving rise to $\rho$. Finally, let $\jnst'$ be $\core \circ \trim_N \circ \unfold(\chase{\inst', \rsd})$. 
    
    If $|P_t| > n$ then for every words $w, w'$ the term $wtw'$ of $\unfold(\chase{\inst', \rsd})$ will be removed by $\trim_N$ function if it exists, due to it having no label. Thus $h$ can serve as a homomorphism from $\jnst'$ to $\map$. 
    
    Assume $|P_t| \leq n$. Let $u$ denote  term of $\jnst$ and let $u'$ denote $\word(P_t)\word(P)t'$. Note that by the definitions of $\core, \trim$, $\unfold$ operations and thanks to rules of $\rsd$ such $u$ exists. If $u'$ does not exists then 
    
    
    As $u$ is at depth $d \leq n$ Property~\ref{map:shallow-compliance} of the map can be applied. Let $w = \pair{h, u', u_+}$ be the $(k \rightarrow \kp)$-compliance witness for $u$. We want to construct a basis $\inst_+$ for the required $\inst'$. To do that we take $\inst_0$ and consecutively copy labels from the path from $u$ to $u_+$ over the elements of $P_+$. We set $\inst_{+}$ to be the resulting instance. Thanks to Properties~\ref{map:embedding-and-unfolding} and ~\ref{map:modelhood} of the map, and the existence of $w$ it should be clear that $\core \circ \trim_N \circ \unfold(\inst_+)$ homomorphically maps to map $\map$. Again, such constructed $\inst_+$ will serve us as a basis for $\inst'$.

First note, that the depth-labels over $P_+$ are the same in any element of $\iter(\inst, \pi)$. This is thanks to (\ref{tag:depths-closure}) and (\ref{tag:depths-propagation}) rules of $\rsp$. Thus from Property \ref{map:minimality} of the map the same labels as on path from $u$ to $u_+$ can be ``guessed'' by $\rsp$. Observe that in $\iter(\inst, \pi)$ there is only one such instance - as the only disjunctive rules of $\rsp$ are those guessing the labels of terms. Thus, instances $\inst_{+}$ and $\inst_{\iter}$ can in principle differ only by a special, single atom, namely $\goal(a)$. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OLDER STUFF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





    
    
    $t$ has no label and thus for every words $w$, $w'$ the terms $wtw'$ will be removed by trim function in  $\core \circ \trim_N \circ \unfold(\chase{\inst', \rsd})$
    
    it will be removed by $\trim$ function along with any terms reachable from it including new elements  there are no atoms over $t$

If $t$ has no label then it appears in the chase at depth greater than $n$. Therefore, the observation holds trivially as all successors of $t$ including all new elements of $P'$ are removed by $\trim$ function before homomorphic mapping is considered, thus the homomorphism from assumption can be reused.

Assume that $t$ has a label, and thus is at depth $d \leq n$.
Let $u'$ be the term of $\jnst$ such that the shortest path from the minimal (recall Observation~\ref{obs:chase-has-minimal}) term of $\inst$ to $t'$ is isomorphic to the path from the root of $\jnst$ to $u'$, and let $u$ be the predecessor of $u'$ at distance $k$ from $u$. Note that by the definitions of $\core, \trim$, and $\unfold$ operations such $u$ and $u'$ exist. Let $h$ be the homomorphism from $\jnst$ to $\map$ and let $v = h(u), v' = h(u')$.

As $u$ is at depth $d$ Property~\ref{map:shallow-compliance} of the map can be applied. Let $w = \pair{h, u', u_+}$ be the $(k \rightarrow \kp)$-compliance witness for $u$. We want to construct a basis $\inst_+$ for the required $\inst'$. To do that we take $\inst_0$ and consecutively copy labels from the path from $u$ to $u_+$ over the elements of $P_+$. We set $\inst_{+}$ to be the resulting instance. Thanks to Properties~\ref{map:embedding-and-unfolding} and ~\ref{map:modelhood} of the map, and the existence of $w$ it should be clear that $\core \circ \trim_N \circ \unfold(\inst_+)$ homomorphically maps to map $\map$. Again, such constructed $\inst_+$ will serve us as a basis for $\inst'$.

First note, that the depth-labels over $P_+$ are the same in any element of $\iter(\inst, \pi)$. This is thanks to (\ref{tag:depths-closure}) and (\ref{tag:depths-propagation}) rules of $\rsp$. Thus from Property \ref{map:minimality} of the map the same labels as on path from $u$ to $u_+$ can be ``guessed'' by $\rsp$. Observe that in $\iter(\inst, \pi)$ there is only one such instance - as the only disjunctive rules of $\rsp$ are those guessing the labels of terms. Thus, instances $\inst_{+}$ and $\inst_{\iter}$ can in principle differ only by a special, single atom, namely $\goal(a)$. 
    
\end{proof}

We shall prove the following, which applied inductively grants us Lemma~\ref{lem:map-to-chase}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OLDEST STUFF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{comment}


Given an instance $\inst$ and any trigger $\pi$ of $\rsa$ in $\inst$ let $\iter(\inst, \pi)$ denote the set of instances resulting from the application of the following two-part operation: 

\begin{enumerate}
    \item Apply $\pi$.
    \item Saturate with rule applications of Datalog rules of $\rsp$.
\end{enumerate}

\noindent
Given an instance $\inst$ and any trigger $\pi$ of some non-Datalog rule of $\rsp$ in $\inst$ let $\iterr(\inst, \pi)$ denote the set of instances resulting from the application of the following two-part operation: 

\begin{enumerate}
    \item Apply $\pi$.
    \item Saturate with rule applications of Datalog rules of $\rsp$.
\end{enumerate}

First note that any chase of $\chases$ can be obtained by looping the following two operations and selecting an element of the resulting set each time.

\begin{lemma}\label{obs:proof-of-main-lema-a}
Given an instance $\inst$ and a map $\map$
if $\core \circ \trim_N \circ \unfold(\inst)$ homomorphically maps to $\map$ then for every $\rsa$-trigger $\pi$ in $\inst$ there exists $\inst' \in \iter(\inst, \pi)$ such that $\core \circ \trim_N \circ \unfold(\inst')$ homomorphically maps to $\map$.

\end{lemma}
\begin{proof}

Let $\jnst = \core \circ \trim_N \circ \unfold(\inst)$. Then let $\inst_{0}$ to be the result of applying $\pi$,  $P$ be the path from $t$ to $t'$ witnessing that $\pi$ was not satisfied in $\inst$, and $P_+$ be the freshly created path. Finally let $k \rightarrow \kp$ be the existential rule of $\pi$.

If $t$ has no label then it appears in the chase at depth greater than $n$. Therefore, the observation holds trivially as all successors of $t$ including all new elements of $P'$ are removed by $\trim$ function before homomorphic mapping is considered, thus the homomorphism from assumption can be reused.

Assume that $t$ has a label, and thus is at depth $d \leq n$.
Let $u'$ be the term of $\jnst$ such that the shortest path from the minimal (recall Observation~\ref{obs:chase-has-minimal}) term of $\inst$ to $t'$ is isomorphic to the path from the root of $\jnst$ to $u'$, and let $u$ be the predecessor of $u'$ at distance $k$ from $u$. Note that by the definitions of $\core, \trim$, and $\unfold$ operations such $u$ and $u'$ exist. Let $h$ be the homomorphism from $\jnst$ to $\map$ and let $v = h(u), v' = h(u')$.

As $u$ is at depth $d$ Property~\ref{map:shallow-compliance} of the map can be applied. Let $w = \pair{h, u', u_+}$ be the $(k \rightarrow \kp)$-compliance witness for $u$. We want to construct a basis $\inst_+$ for the required $\inst'$. To do that we take $\inst_0$ and consecutively copy labels from the path from $u$ to $u_+$ over the elements of $P_+$. We set $\inst_{+}$ to be the resulting instance. Thanks to Properties~\ref{map:embedding-and-unfolding} and ~\ref{map:modelhood} of the map, and the existence of $w$ it should be clear that $\core \circ \trim_N \circ \unfold(\inst_+)$ homomorphically maps to map $\map$. Again, such constructed $\inst_+$ will serve us as a basis for $\inst'$.

First note, that the depth-labels over $P_+$ are the same in any element of $\iter(\inst, \pi)$. This is thanks to (\ref{tag:depths-closure}) and (\ref{tag:depths-propagation}) rules of $\rsp$. Thus from Property \ref{map:minimality} of the map the same labels as on path from $u$ to $u_+$ can be ``guessed'' by $\rsp$. Observe that in $\iter(\inst, \pi)$ there is only one such instance - as the only disjunctive rules of $\rsp$ are those guessing the labels of terms. Thus, instances $\inst_{+}$ and $\inst_{\iter}$ can in principle differ only by a special, single atom, namely $\goal(a)$. 

There are four cases depending of whether $\goal(a)$ is present in map $\map$ and whether it is was just derived in $\inst_\iter$. If $\goal(a) \in \map$ then no matter whether $\goal(a) \in \inst_\iter$ or not, $\inst_\iter$ is homomorphically mappable to $\map$ and thus it can serve as $\inst'$.

Assume that $\goal(a) \not\in \map$. If $\inst_\iter$ does not contain $\goal(a)$ then it is homomorphically mappable to $\map$ as $\inst_{+}$ is. Thus $\inst_\iter$ can serve as $\inst'$.

Finally assume that $\goal(a) \not \in \map$ but $\goal(a) \in \inst_\iter$. However, note that $\chase{\inst_0, \rsp} = \inst_\iter$, $\map$ is a model of $\rsp$, and $\spairs(\inst_0) \subseteq \spairs(\map)$, but $\goal(a) \not \in \map$. This is a contradiction by \piotr{Lemma stating that violations of modelhood of $\rsp$ can be witnessed by a single spair.}
\end{proof}

The following is proven analogously:

\begin{observation}\label{obs:proof-of-main-lema-b}
Given an instance $\inst$ and a map $\map$
if $\core \circ \trim_N \circ \unfold(\inst)$  homomorphically maps to $\map$ then for every non-Datalog trigger $\pi$ of $\rsp$ in $\inst$ there exists $\inst' \in \iter(\inst, \pi)$ such that $\core \circ \trim_N \circ \unfold(\inst')$ homomorphically maps to $\map$.
\end{observation}
\begin{proof}
\piotr{TODO if time - this one is boring.}

One can inductively combine the above to obtain Lemma~\ref{lem:map-to-chase}.

\end{proof}
\end{comment}

==> other/log-prelims.tex <==


\subsection{Logical Preliminaries}


In this section, we introduce the language, semantics, and axiomatization for the intuitionistic modal logic $\ik$~\cite{PloSti86}.\footnote{See Simpson's 1994 PhD Thesis~\cite{Sim94} for a detailed introduction and discussion of $\ik$.} Moreover, we also introduce extensions of $\ik$ (referred to as \emph{intuitionistic modal logics} more generally) with the seriality axiom $\axd$ and axioms that we refer to as \emph{Horn-Scott-Lemmon Axioms ($\axhsl$s)}.

We define our intuitionistic modal language $\lang$ to be the set of formulae generated via the following BNF grammar:
$$
A ::= p \ | \ \bot \ | \ A \lor A \ | \ A \land A \ | \ A \iimp A \ | \ \dia A \ | \ \Box A
$$
where $p$ ranges over the set of propositional atoms $\prop := \{p, q, r, \ldots\}$. We use $A$, $B$, $C$, \etc (occasionally annotated) to range over formulae in $\lang$, and define $\inot A := A \iimp \bot$ and $A \ieq B := (A \iimp B) \land (B \iimp A)$. For $n \in \mathbb{N}$, we use $\dia^{n} A$ and $\Box^{n} A$ to represent the formula $A$ prefixed with a sequence of $n$ diamonds or boxes, respectively. We interpret such formulae on \emph{bi-relational models}~\cite{PloSti86,Sim94}: 

%Pg. 50 of Simpson
\begin{definition}[Bi-relational Model~\cite{PloSti86}]\label{def:bi-relational-model} We define a \emph{bi-relational model} to be a tuple $M := (W, \leq, R, V)$ such that:
\begin{itemize}

\item $W$ is a non-empty set of \emph{worlds} $w, u, v, \ldots$ (potentially annotated);

\item The \emph{intuitionistic relation} $\leq \ \subseteq W \times W$ is %a preorder, i.e. it is 
 reflexive and transitive;

\item The \emph{accessibility relation} $R \subseteq W \times W$ satisfies:

\begin{itemize}

\item[(F1)] For all $w, v, v' \in W$, if $w R v$ and $v \leq v'$, then there exists a $w' \in W$ such that $w \leq w'$ and $w' R v'$;

\item[(F2)] For all $w, w', v \in W$, if $w \leq w'$ and $w R v$, then there exists a $v' \in W$ such that $w' R v'$ and $v \leq v'$;

\end{itemize}

%\item For the set $\fworlds \subseteq W$ of \emph{fallible worlds}, if $w \in \fworlds$, and $wR_{\charx}u$ or $w \leq u$, then $u \in \fworlds$.

\item $V : W \to 2^{\prop}$ is a \emph{valuation function} satisfying the \emph{monotonicity condition}:  For each $w, u \in W$, if $w \leq u$, then $V(w) \subseteq V(u)$.

\end{itemize}

\end{definition}

%The (F1) and (F2) conditions can be visualized with the respective diagrams below. The dotted edges are those that are taken to exist given that the solid edges exist in a bi-relational model.

%\begin{center}
%\begin{tabular}{c @{\hskip 3em} c}
%\xymatrix{
% w'\ar@{.>}[rr]^{R}  & & v'   \\
% w\ar@{.>}[u]^{\leq}\ar[rr]_{R} &  & v\ar[u]_{\leq}
%}

%&

%\xymatrix{
% w'\ar@{.>}[rr]^{R} &  & v' \\
%w\ar[u]^{\leq}\ar[rr]_{R} & & v\ar@{.>}[u]_{\leq}
%}

%\end{tabular}
%\end{center}


Formulae from $\lang$ may then be interpreted over bi-relational models as specified by the semantic clauses below. %We note that in the intuitionistic setting the $\dia$ and $\Box$ modalities fail to be interdefinable (i.e. they fail to be dual to one another), that is, $\dia A \ieq \inot \Box \inot A$ is not valid according to the semantics for intuitionistic modal logics. This break down in the interdefinability of $\dia$ and $\Box$ is similar to the well-known fact that $\lor$ and $\land$, and $\exists$ and $\forall$, fail to be interdefinable in (first-order) intuitionistic logic.


%\cite{GabSheSkv09}
\begin{definition}[Semantic Clauses~\cite{PloSti86}]
\label{def:semantic-clauses} Let $M$ be a bi-relational model with $w \in W$ of $M$. The \emph{satisfaction relation} $M,w \Vdash A$ %between $w$ and a formula $A \in \lang$ 
 is defined recursively:

\begin{itemize}

\item $M,w \Vdash p$ \ifandonlyif $p \in V(w)$, for $p \in \prop$;

\item $M, w \not\Vdash \bot$;

\item $M,w \Vdash A \lor B$ \ifandonlyif $M,w \Vdash A$ or $M,w \Vdash B$;

\item $M,w \Vdash A \land B$ \ifandonlyif $M,w \Vdash A$ and $M,w \Vdash B$;

\item $M,w \Vdash A \iimp B$ \ifandonlyif for all $w' \in W$, if $w \leq w'$ and $M,w' \Vdash A$, then $M,w' \Vdash B$;

\item $M,w \Vdash \dia A$ \ifandonlyif there exists a $v \in W$ such that $w R v$ and $M,v \Vdash A$;

\item $M,w \Vdash \Box A$ \ifandonlyif for all $w', v' \in W$, if $w \leq w'$ %, then for all $v' \in W$, if 
 and $w' R v'$, then $M,v' \Vdash A$.

\end{itemize}
We say that a formula $A$ is \emph{globally true on $M$}, written $M \Vdash A$, \ifandonlyif $M,u \Vdash A$ for all worlds $u \in W$ of $M$, and we say that a formula $A$ is \emph{valid}, written $\Vdash A$, \ifandonlyif $A$ is globally true on all bi-relational models.
\end{definition}


As shown by Plotkin and Stirling in~\cite{PloSti86}, the validities of $\ik$ are axiomatizable:


%Pg. 52 Simpson
\begin{definition}[Axiomatization~\cite{PloSti86}] We define the axiomatization $\h\ik$ as:

%\begin{multicols}{2}
\begin{itemize}

\item[A0] Axioms for propositional intuitionistic logic~\cite{?}

\item[A1] $\Box (A \iimp B) \iimp (\Box A \iimp \Box B)$

\item[A2] $\Box (A \iimp B) \iimp (\dia A \iimp \dia B)$

\item[A3] $\inot \dia \bot$

\item[A4] $\dia (A \lor B) \iimp (\dia A \lor \dia B)$

\item[A5] $(\dia A \iimp \Box B) \iimp \Box (A \iimp B)$

\item[R0] \AxiomC{$A$}\AxiomC{$A \iimp B$}\RightLabel{(mp)}\BinaryInfC{$B$}\DisplayProof

\item[R1] \AxiomC{$A$}\RightLabel{(nec)}\UnaryInfC{$\Box A$}\DisplayProof

\end{itemize}
%\end{multicols}
We define $\ik$ to be the smallest set of formulae closed under substitutions of the above axioms and applications of the inference rules, and define $A$ to be a \emph{theorem} of $\ik$ \ifandonlyif $A  \in \ik$.
\end{definition}

%Pg. 107 Simpson for Axioms and Frame Properties
We also consider %logics generated by 
 extensions of $\h\ik$ with sets $\axs$ of the following axioms:
$$
\axd: \Box A \iimp \dia A \quad \axhsl: (\dia^{n} \Box A \iimp \Box^{k} A) \land (\dia^{k} A \iimp \Box^{n} \dia A)
$$
The above left axiom is referred to as the \emph{seriality axiom $\axd$} and axioms of the form above right are referred to as \emph{Horn-Scott-Lemmon axioms ($\axhsl$s)}, which we use $\gmp$ to denote.\footnote{We note that the term \emph{Horn-Scott-Lemmon axiom} arises from the fact that such axioms form a proper subclass of the well-known \emph{Scott-Lemmon Axioms}~\cite{Lem77} and are associated with frame conditions that are expressible as Horn formulae~\cite[\sect~7.2]{Sim94}.} For the remainder of the paper, we use $\axs$ to denote an arbitrary set of the above axioms, that is:
$$
\axs \subseteq \{\axd\} \cup \{(\dia^{n} \Box A \iimp \Box^{k} A) \land (\dia^{k} A \iimp \Box^{n} \dia A) \ | \ n,k \in \mathbb{N} \}
$$
The set of $\axhsl$s includes well-known axioms such as:
%Below are given on Pg. 56 of Simpson
$$
\axt: (A \iimp \dia A) \land (\Box A \iimp A) \quad
\axfour: (\dia \dia A \iimp \dia A) \land (\Box A \iimp \Box \Box A)
$$
$$
\axb: (\dia \Box A \iimp A) \land (A \iimp \Box \dia A) \quad
\axfive: (\dia \Box A \iimp \Box A) \land (\dia A \iimp \Box \dia A)
$$
The work of Simpson~\cite{Sim94} establishes that any extension of $\h\ik$ with a set $\axs$ of axioms is sound and complete relative to a subclass of the bi-relational models. In particular, the extension of $\h\ik$ with a set $\axs$ of axioms is sound and complete relative to the set of bi-relational models satisfying the frame conditions related to the axioms of $\axs$, as specified in \fig~\ref{fig:axioms-related-conditions}.\footnote{We note that the axioms we consider do not \emph{characterize} the set of frames satisfying the frame properties related to the axioms as they do in the classical setting. For more details concerning this point, see~\cite[p.~56]{Sim94}, and for details concerning the proper characterization results of the above axioms, see~\cite{PloSti86}.} We define axiomatic extensions of $\h\ik$ along with their corresponding models below:

\begin{figure}[t]
\begin{center}
\bgroup
\def\arraystretch{1.1}
\begin{tabular}{| l | l |}
\hline
Axiom & Frame Condition\\
\hline
$\Box A \iimp \dia A$ & $\forall w \exists u (w R u)$\\
%\hline
$(\dia^{n} \Box A \iimp \Box^{k} A) \land (\dia^{k} A \iimp \Box^{n} \dia A)$ & $\forall w, u, v (w R^{n} u \land w R^{k} v \iimp u R v)$\\
\hline
\end{tabular}
\egroup
\end{center}

\caption{Axioms and their related frame conditions. We note that when $n=0$, the related frame condition is $\forall w, v (w R^{k} v \iimp w R v)$, when $k = 0$, the related frame condition is $\forall w, u (w R^{n} u \iimp u R w)$, and when $n = k = 0$, the related frame condition is $\forall w (w R w)$.}
\label{fig:axioms-related-conditions}
\end{figure}

\begin{definition}[Extensions, Bi-relational $\axs$-model, $\axs$-valid] The axiomatization $\h\ik(\axs)$ is defined to be $\h\ik$ extended with the axioms from $\axs$, and we define the \emph{logic} $\ika$ to be the smallest set of formulae closed under substitutions of the axioms of $\h\ika$ and applications of the inference rules. Also, a \emph{theorem} of $\ika$ is a formula $A$ such that $A \in \ika$. Moreover, we define a \emph{bi-relational $\axs$-model} to be a bi-relational model satisfying each frame condition related to an axiom $A \in \axs$ (as specified in \fig~\ref{fig:axioms-related-conditions}). Last, a formula $A$ is \emph{$\axs$-valid} \ifandonlyif it is globally true on all $\axs$-models.
\end{definition}

\begin{remark} We note that $\h\ik = \h\ik(\emptyset)$ and that a bi-relational $\emptyset$-model is a bi-relational model.
\end{remark}

%Pg. 107 Thm 6.2.1 of Simpson says "A is a theorem of IK + Axioms iff A is a theorem NDIK + Axioms", Pg. 78 has soundness Thm 4.8.1, and Pg. 89 should have compelteness expressed in Thm. 5.2.1 or Pg 86 with Thm. 5.1.1
%Thm 8.1.4 on Pg. 156 gives a type of completeness and soundness for extensions of the ND IK system
%Pg. 107 Simpson, but need to find explicit statement of this fact
\begin{theorem}[Soundness and Completeness~\cite{Sim94}]\label{thm:sound-complete-ikma}
A formula is a theorem of $\h\ika$ \ifandonlyif it is valid in all $\axs$-frames.
\end{theorem}

\begin{IEEEproof}
Follows from \thm~6.2.1 and \thm~8.1.4 of~\cite{Sim94}.
\end{IEEEproof}



\subsection{Grammar-theoretic Preliminaries}



As will be seen later on (viz. in \sect~\ref{sec:refinement} and~\ref{sec:nested-calculi}), a central component to our refinement methodology---i.e. the extraction of nested calculi from labelled---is the use of inference rules whose applicability is determined on the basis of strings generated by a formal grammar. We therefore introduce grammar-theoretic notions that are essential to the functionality of such rules.

We let $\albet$ be our \emph{alphabet} consisting of the \emph{characters} $\fd$ and $\bd$, that is, $\albet := \{\fd,\bd\}$. The symbols $\fd$ and $\bd$ will be used to encode information about the accessibility relation $R$ of a bi-relational model in certain inference rules of our calculi. In particular, $\fd$ will be used to encode information about what is happening in the \emph{future} of the accessibility relation, and $\bd$ will be used to encode information about what is happening in the \emph{past} of the accessibility relation. We note that such symbols have been chosen due to their analogous meaning in the context of tense logics~\cite{GorPosTiu11,Kas94}. Also, following~\cite{GorPosTiu11}, we let $\ques \in \albet$ and $\conv{\ques} \in \albet \setminus \{\ques\}$, i.e. $\conv{\fd} := \bd$ and $\conv{\bd} := \fd$; we refer to $\fd$ and $\bd$ as \emph{converses} of one another. We may define \emph{strings} over our alphabet $\albet$ accordingly:

%~\cite{DemNiv05}
\begin{definition}[$\albetstr$] We let $\concat$ be the \emph{concatenation operation} with $\varepsilon$ the \emph{empty string}. We define the set $\albet^{*}$ of \emph{strings over $\albet$} to be the smallest set such that:
\begin{itemize}

\item $\albet \cup \{\varepsilon\} \subseteq \albet^{*}$

\item $\text{If } \stra \in \albet^{*} \text{ and } \ques \in \albet \text{, then } \stra \concat \ques \in \albet^{*}$

\end{itemize}
\end{definition}

For a set $\albetstr$ of strings, we use $\stra$, $\strb$, $\strc$, \etc (potentially annotated) to represent strings in $\albetstr$. Also, the empty string $\empstr$ is taken to be the identity element for the concatenation operation, i.e. $\stra \concat \empstr = \empstr \concat \stra = \stra$ for $\stra \in \albet^{*}$. Furthermore, we will not explicitly mention the concatenation operation in practice and let $\stra \cate \strb := \stra \concat \strb$, that is, we denote concatenation by simply gluing two strings together. Beyond concatenation, another useful operation to define on strings is the \emph{converse operation}, adapted from~\cite{TiuIanGor12}.

\begin{definition}[String Converse] We extend the converse operation to strings as follows:
\begin{itemize}

\item $\conv{\varepsilon} := \varepsilon$;

\item $\text{If } \stra = \ques_{1} \cdots \ques_{n} \text{, then } \conv{\stra} := \conv{\ques}_{n} \cdots \conv{\ques}_{1}$.

\end{itemize}
\end{definition}


%\begin{definition}[String Length] The \emph{length} of a string $\stra \in \albet^{*}$ is defined recursively: 
%\begin{itemize}

%\item $\lenstr{\stra} := 0$, if $\stra = \empstr$;

%\item $\lenstr{\stra} = \lenstr{\strb \cate \ques} := \lenstr{\strb} + 1$, if $\stra = \strb \cate \ques$ with $\strb \in \albet^{*}$ and $\ques \in \albet$.

%\end{itemize}
%\end{definition}

We let $\ques^{n}$ denote a string consisting of $n$ copies of $\ques$, which is $\empstr$ when $n = 0$. Making use of such notation, we can compactly define the notion of an \emph{$\axs$-grammar}, which encodes information contained in a set $\axs$ of axioms, and which will be employed in the definition of certain inference rules (see \sect~\ref{sec:refinement}).


\begin{definition}[$\axs$-grammar]\label{def:grammar} We define an \emph{$\axs$-grammar} to be a set $\g{\axs}$ such that:
\begin{center}
$(\dia \pto \bd^{n} \cate \dia^{k}), (\bd \pto \bd^{k} \cate \fd^{n}) \in \g{\axs}$ \ifandonlyif $(\dia^{n} \Box A \iimp \Box^{k} A) \land (\dia^{k} A \iimp \Box^{n} \dia A) \in \axs$.
\end{center}
We call rules of the form $\ques \pto \stra$ \emph{production rules}, where $\ques \in \albet$ and $\stra \in \albetstr$.
\end{definition}



%\begin{figure}[t]
%\begin{center}
%\bgroup
%\def\arraystretch{1.1}
%\begin{tabular}{| l | l | l |}
%\hline
%Name & Frame Property & Production Rules\\
%\hline
%Reflexivity & $\forall w wRw$ & $\{\ques \pto \empstr \ | \ \ques \in \albet\}$ \\
%Symmetry & $\forall w, u (wRu \iimp uRw)$ & $\{\ques \pto \conv{\ques} \ | \ \ques \in \albet\}$ \\
%Transitivity & $\forall w, v, u (wRv \land vRu \iimp wRu)$ & $\{\ques \pto \ques \cate \ques \ | \ \ques \in \albet\}$ \\
%Euclideanity & $\forall w, v, u (wRv \land wRu \iimp vRu)$ & $\{\ques \pto \conv{\ques} \cate \ques \ | \ \ques \in \albet\}$ \\
%\hline
%\end{tabular}
%\egroup
%\end{center}
%\caption{**double check these}
%\label{fig:frame-conditions-production-rules}
%\end{figure}



An $\axs$-grammar $\g{\axs}$ is a type of \emph{Semi-Thue system} (cf.~\cite{Pos47}), i.e. it is a string re-writing system. For example, assuming that $\ques \pto \stra \in \g{\axs}$, we may derive the string $\strb \cate \stra \cate \strc$ from $\strb \cate \ques \cate \strc$ in one-step by applying the mentioned production rule. As usual, through successive applications of production rules to a string $\stra \in \albetstr$, one obtains derivations of new strings, the collection of which, determines a language. We make such notions precise by means of the following definition:


%~\cite{DemNiv05}
\begin{definition}[Derivation, Language]\label{def:derivation-language} Let $\g{\axs}$ be an $\axs$-grammar. The \emph{one-step derivation relation} $\osdr$ holds between two strings $\stra$ and $\strb$ in $\albetstr$, written $\stra \osdr \strb$, \ifandonlyif there exist $\stra', \strb' \in \albetstr$ and $\ques \pto \strc \in \thuesys$ such that $\stra = \stra' \cate \ques \cate \strb'$ and $\strb = \stra' \cate \strc \cate \strb'$.  The \emph{derivation relation} $\dr$ is defined to be the reflexive and transitive closure of $\osdr$. For two strings $\stra, \strb \in \albetstr$, we refer to $\stra \dr \strb$ as a \emph{derivation of $\strb$ from $\stra$}, and define its \emph{length} to be equal to the minimal number of one-step derivations needed to derive $\strb$ from $\stra$ in $\g{\axs}$. Last, for a string $\stra \in \albet^{*}$, the \emph{language of $\stra$ relative to $\g{\axs}$} is defined to be the set $\glang(\stra) := \{\strb \ | \ \stra \dr \strb \}$.
\end{definition}







==> other/notation.tex <==
%PACKAGES
\usepackage{amssymb, amsmath, mathrsfs}
\usepackage{synttree, bussproofs,scrextend, stmaryrd, rotating, xcolor, algorithmicx, upgreek}
\usepackage{algorithm}% http://ctan.org/pkg/algorithms
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
\usepackage{esvect,pgf, tikz, color}
\usetikzlibrary{arrows, automata}
\usepackage[all]{xy}
\usepackage{changepage,enumerate,proof,upgreek,relsize,trfsigns,
comment}
\usepackage{multicol}

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

% Theorem, Lemma, etc
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}


%%%ENVIROMENTS
\newtheorem{innercustomlem}{Lemma}
\newenvironment{customlem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomlem}
  
  \newtheorem{innercustomthm}{Theorem}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
  
\newtheorem{innercustomprop}{Proposition}
\newenvironment{customprop}[1]
  {\renewcommand\theinnercustomprop{#1}\innercustomprop}
  {\endinnercustomprop}
  
\newtheorem{innercustomcor}{Corollary}
\newenvironment{customcor}[1]
  {\renewcommand\theinnercustomcor{#1}\innercustomcor}
  {\endinnercustomcor}
  
\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}


\def\phi{\varphi}

%%%Colors and comments for notes, changes, etc.
\definecolor{tim}{RGB}{0, 0, 250}
\newcommand{\tim}[1]{\textbf{\textcolor{black}{tim}}: {\color{tim}#1}}


%%%ABBREVIATIONS
\newcommand{\ifandonlyif}{\textit{iff} }
\newcommand{\iffi}{\textit{iff} }
\newcommand{\etc}{$\ldots$ }
\newcommand{\dfn}{Definition}
\newcommand{\fig}{Figure}
\newcommand{\lem}{Lemma}
\newcommand{\thm}{Theorem}
\newcommand{\prp}{Proposition}
\newcommand{\ih}{IH}
\newcommand{\sect}{Section}
\newcommand{\cptr}{Ch.}

%%%Sequent Notation
\newcommand{\sar}{\vdash}
\newcommand{\bl}{[}
\newcommand{\br}{]}
\newcommand{\sbl}{\{}
\newcommand{\sbr}{\}}


%%%Proof System Notation
\newcommand{\prf}{\mathcal{D}}


